Answering Regular Path Queries on Workflow Provenance

This paper proposes a novel approach for efficiently evaluating regular path queries over provenance graphs of workflows that may include recursion. The approach assumes that an execution g of a workflow G is labeled with query-agnostic reachability labels using an existing technique. At query time, given g, G and a regular path query R, the approach decomposes R into a set of subqueries R1, ..., Rk that are safe for G. For each safe subquery Ri, G is rewritten so that, using the reachability labels of nodes in g, whether or not there is a path which matches Ri between two nodes can be decided in constant time. The results of each safe subquery are then composed, possibly with some small unsafe remainder, to produce an answer to R. The approach results in an algorithm that significantly reduces the number of subqueries k over existing techniques by increasing their size and complexity, and that evaluates each subquery in time bounded by its input and output size. Experimental results demonstrate the benefit of this approach.

==> outline.tex <==
\section{Paper Outline}
\label{sec:outline}

\subsection{Pairwise Queries}
We start by considering "pairwise" regular path queries. That is, given two nodes (of an execution) and a regular expression, we want to decide if there is a path connecting two nodes such that the path label (i.e., the sequence of edge labels on this path) matches the given regular expression.

We show that for a natural class of "safe" combinations of workflow specifications (grammars) and regular expressions, the "pairwise" regular path queries can be \eat{efficiently} answered using the skeleton-based labeling approach in {\em constant} time if the grammar is fixed. Note that existing lableing schemes for trees or graphs are designed for answering reachability queries rather than regular path queries. It is unknown if it is possible to answer pairwise regular path queries over trees or graphs in constant time. 

In the rest of the paper, we will reuse notions in \cite{DBLP:conf/sigmod/BaoDM12}, such as strictly linear recursive grammars, production graph, compressed parse tree. Recall that a workflow grammar $G$ is said to be strictly linear-recursive if all the cycles in its production graph are vertex-disjoint. 

\eat{
\begin{definition}
\textbf{(Production Graph)} Given a workflow grammar $G=(\Sigma,\Delta, S,P)$, the production graph of $G$ is a directed multigraph ${\cal  P}(G)$ in which each vertex denotes a unique module in $\Sigma$. For each production $M\rightarrow W$ in $P$ and each module $M'\in W$, there is an edge from $M$ to $M'$ in ${\cal P}(G)$. Note that if $W$ has multiple instances of a module $M'$, then ${\cal P}(G)$ has multiple parallel edges from $M$ to $M'$.
\end{definition}}


\begin{definition}
\textbf{(Safety)} Given a workflow specification $G$ and a regular expression $R$, for each composite module $C$ in $G$, let $f_C$ be a mapping from $Q \times Q$ to $\{ 0, 1 \}$, where $Q$ is the set of states of the automaton accepting $R$. Moreover, $f_C(q, q') = 1$ iff there is a path from the input of $C$ to the output of $C$ and when the automaton reads this path, its state transits from $q$ to $q'$. Then $(G, R)$ is said to be safe if for every composition module C, $f_C$ is unique for all possible executions of $C$.
\end{definition}

\begin{theorem}
Given a strictly linear-recursive workflow grammar $G$, for any safe regular path query $R$ w.r.t. $G$, there is a compact and efficient dynamic labeling scheme for $G$.
\end{theorem}

\subsection{All-pairs Queries}
We next turn to "allpairs" regular path queries. That is, given a regular expression, we want to find all pairs of nodes for which there is a connecting path whose label matches the given regular expression.

A naive approach: recall that a regular expression is built by three constructs: concatenation, alternation, and Kleene star. The concatenation can be evaluated by testing the adjacency of the two lists of nodes (or node pairs), called adjacent-join. The alternation can be evaluated by taking the union of two lists of nodes (or node pairs). The Kleene star can be evaluated by computing a fixed point of repeated concatenation.

Our problem: How to optimize the evaluation of "allpairs" regular path queries?

Our approach: We want to minimize the above expensive computation (using the naive approach) by decomposing the given regular expression into a set of sub-expressions. Among them, some are safe sub-expressions (with respect to the given workflow specification), which can be efficiently evaluated using the labeling, the others are unsafe sub-expressions, which have to be evaluated using the naive approach. Note that the existing index approach can also be used to improve the unsafe sub-expressions.

Algorithm sketch:

Case 1: we first consider a simple case, where the given regular expression has only concatenation (but no alternation nor Kleene star). We compute the best partition of the regular expression using a dynamic programming.

Case 2: We next consider a more complex case, where the given regular expression has only concatenation and Kleene star (but no alternation). Consider the parse tree of the given regular expression. We use a dynamic programming to the compute the best plan for each sub-tree in a bottom-up manner. For each subtree, we compute the best partition of the children of the root again using a dynamic programming as Case 1.

Case 3: For the general case which involves all the three constructs, we need to all possible equivalent rewrites of the given regular expression by expanding the alternation. The number of possible rewrite can be exponential. (If we do not consider regular expression rewriting, we can use the approach in Case 2 to solve the general case.)

\subsection{Main Results}\label{main_results}
%Main results of this paper are shown in Figure~\ref{queries} and \ref{allpairs-queries}.
Related work and main results (shadowed) of this paper are shown in Figure~\ref{queries} and Figure~\ref{allpairs-queries}.

\begin{figure}[h]
\centering
\includegraphics[scale=0.6]{docs/queries-crop.pdf}
\caption{Dynamic Labeling Schemes for Pairwise Queries}
\label{queries}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[scale=0.62]{docs/allpairsQueries-crop.pdf}
\caption{Query Time for All-pairs Queries}
\label{allpairs-queries}
\end{figure}

\eat{
\begin{figure*}
\begin{tabular}{|l l|l|l|l|l|l|} \hline
\multicolumn{2}{|c|}{\multirow{3}{*}{Workflows}}& Reachability&\multicolumn{2}{|c|}{Regular Queries}&\multicolumn{2}{|c|}{Regular Queries}\\
						 &&Queries & \multicolumn{2}{|c|}{(pair-wise)}& \multicolumn{2}{|c|}{(all-pairs)}\\\cline{4-7}
						 &&(pair-wise)&safe&unsafe&safe&unsafe \\ \hline
\multirow{4}{*}{\small Coarse-grained} & strictly linear recursions &\multirow{2}{*}{$\shortstack{\text{\small Compact labeling scheme}\\ \text{constant query time}}$}& $\substack{\text{Compact labeling scheme}\\ \text{constant query time}}$&&$\substack{\text{Compact labeling scheme}\\ \text{linear query time}}$&\\[8ex] \cline{4-4}\cline{6-6}
				& linear recursions&\\ \cline{2-3}
				& arbitrary workflows &linear-size labeling\\\cline{2-3}
&arbitrary DAGs&
\\ \hline
\multirow{3}{*}{\small Fine-grained} &strictly linear recursions& $\substack{\text{\small Compact labeling scheme}\\ \text{constant query time}}$\\\cline{2-3}
& linear recursions &\multirow{2}{*}{linear-size labeling}\\
& arbitrary workflows &
\\ \hline
\end{tabular}
\caption{Main Results}
\label{main-result}
\end{figure*}
}

